Code Generation from Natural Language with Less Prior and More Monolingual Data

Training datasets for semantic parsing are typically small due to the higher expertise required for annotation than most other NLP tasks. As a result, models for this application usually need additional prior knowledge to be built into the architecture or algorithm. The increased dependency on human experts hinders automation and raises the development and maintenance costs in practice. This work investigates whether a generic transformer-based seq2seq model can achieve competitive performance with minimal code-generation-specific inductive bias design. By exploiting a relatively sizeable monolingual corpus of the target programming language, which is cheap to mine from the web, we achieved 81.03% exact match accuracy on Django and 32.57 BLEU score on CoNaLa. Both are SOTA to the best of our knowledge. This positive evidence highlights a potentially easier path toward building accurate semantic parsers in practice.

==> background.tex <==
%% <<<<<<< HEAD
%% =======
%% We assume a parallel corpus of natural language utterances and their corresponding programming language codes, $\mathcal{B}=\{\x_i, \y_i\}$.
%% The goal is to train a translator model (TM) to maximize the conditional log probability of $\y_i$ given $\x_i$, $T_{\vtheta}(\y_i|\x_i)$, over the training set:
%% \begin{equation}
%%     \mathcal{L} = \sum_{i} T_{\vtheta}(\y_i \mid \x_i)
%%     \label{eq:objective_conv}
%% \end{equation}
%% \noindent where $\vtheta$ is the vector of TM model parameters.

%% Let $\mathcal{M}=\{\y'_i\}$ denote the monolingual dataset in the target language. Then in the simplest setup, we can train a TM on labeled data $\mathcal{B}$ and a LM on $\mathcal{M}$ independently, and combine the logits of their prediction (potentially weighted) at inference time. This is known as shallow fusion \cite{gulcehre2015using}. One can also share parameters between LM and TM during training \cite{ramachandran2016unsupervised}.

%% %% \begin{equation}
%% %%     \mathcal{L} = E_{p(\x_i, \y_i)} ~ T_{\vtheta}(\y_i \mid \x_i) ~ + ~ \lambda E_{p(\y')} ~ L_{\vtheta}(\y')
%% %%     \label{eq:objective}
%% %% \end{equation}
%% %% Here we augmented the conventional translation objective with a language model (LM) on a monolingual dataset. $\lambda$ controls the balance between the supervised and monolingual sets. 

%% Back-translation \cite{sennrich2015improving}, as the name suggests, trains a translator in the backward direction $q_{\pmb{\phi}}(\x_i | \y_i)$ from target to source sentences using the bitext data $\mathcal{B}$. Then by using this new backward translator we can generate synthetic source sentences in the monolingual set $\y'_i \in \mathcal{M}$, and form a synthetic bitext dataset $\mathcal{B'}=\{\x'_i, \y'_i\}$. This new $\mathcal{B'}$ is combined with the authentic bitext $\mathcal{B}$ to train the TM using Objective \ref{eq:objective_conv}. Several studies \cite{edunov2018understanding, hoang2018iterative} showed that the quality of the synthetic source sentence in the back-translation is crucial to its effectiveness which limits the application in low-resource MT, because the backward translator cannot be well trained at the first place to produce quality synthetic sources.

%% To address this challenge, \cite{currey2017copied, burlot2019using} suggested to copy the target sentences as source ones and demonstrated its effectiveness, essentially adding an auto-encoding objective term on the monolingual data:
%% \begin{equation}
%%     \mathcal{\tilde{L}} = \sum_{\mathcal{B}} T_{\vtheta}(\y_i \mid \x_i) + \sum_{\mathcal{M}} T_{\vtheta}(\y'_i \mid \y'_i)
%% \end{equation}
%% Despite training the encoder using both $\{\x_i\}$ and the target language data points$\{\y'_i\}$, this heuristic proved to be effective in low resource MT.
%% >>>>>>> f26584ae224c3f373a64273e17e77c9b5e82be8d

% Further they claim that this new data has complementary effect to back-translated data. \par
% Most of back-translation approaches merge the synthetic and authentic datasets together and behave them exactly the same. In tagged-back-translation[..] it is argued that by tagging source sentences we avoid the negative effect that some low quality synthetic source can have. Here we follow another direction which is freezing the encoder parameters. 
% and in section 4.1 we compare it against shallow-fusion. 
%  In ablation study 3.1 we compare this to fusion and auxiliary language modeling during training. We also find it helpful to use noisy synthetic source sentences on some datasets which changes the objective to de-noising auto-encoder.



%  \citet{cotterell2018explaining} explains back-translation via wake-sleep where in wake phase we train the backward-translator and in the sleep phase the forward -translator is optimized. This way, you can think of source sentences as latent codes that we marginalize to optimize a lower-bound on the likelihood of target sentences, so back-translation can be perceived as a lowerbound on equation \ref{eq:objective}. However, with extremely limited labeled datasets learning a good back-ward translator is challenging.  
  

